GraphStateVis: Interactive Visual Analysis of Qubit Graph States and their Stabilizer Groups

Fathoming out quantum state space is a challenging endeavor due to its exponentially growing dimensionality. At the expense of being bound in its expressiveness, the discrete and finite subspace of graph states is easier to investigate via a pictorial framework accompanied with a theoretical toolkit from the stabilizer formalism. Analyzing hand-drawn graphs is a tedious and time-consuming task and imposes limitations to the problem sizes that can be addressed. Similarly, algorithmic studies using adjacency matrices alone lack the benefit of a visual representation of the states. We argue that applying visual analytics to investigate graph states can be advantageous. To this end, we introduce GraphStateVis, a web-based application for the visual analysis of qubit graph states and their stabilizer groups. Our tool facilitates the interactive construction of a graph through multiple components supported by linking and brushing. The user can explore graph-state-specific properties, including the Pauli-weight distribution of its stabilizer operators and noise thresholds for entanglement criteria. We propose a use case in the context of near-term quantum algorithms to illustrate the capabilities of our prototype. We provide access to GraphStateVis as an open-source project and invite the broader quantum computing and engineering communities to take advantage of this tool and further boost its development.

==> wrap_figures.tex <==

\newcommand{\vertEdgeContextMenus}{ 
    \begin{wrapfigure}[12]{r}{0.38\columnwidth}
     \vspace{-11pt}
      \begin{center}
        \hspace*{5pt}\includegraphics[width=0.35\columnwidth]{figures/context-menus/context-menus-vert-center.png}
      \end{center}
        \vspace*{-11pt}
      \caption{Context menus for modifying vertices and edges.}
      \label{fig:context-menus}
    \end{wrapfigure}
}
